Interactive Communication for Data Exchange

Two parties observing correlated data seek to exchange their data using interactive communication. How many bits must they communicate? We propose a new interactive protocol for data exchange which increases the communication size in steps until the task is done. Next, we derive a lower bound on the minimum number of bits that is based on relating the data exchange problem to the secret key agreement problem. Our single-shot analysis applies to all discrete random variables and yields upper and lower bound of a similar form. In fact, the bounds are asymptotically tight and lead to a characterization of the optimal rate of communication needed for data exchange for a general sequence such as mixture of IID random variables as well as the optimal second-order asymptotic term in the length of communication needed for data exchange for the IID random variables, when the probability of error is fixed. This gives a precise characterization of the asymptotic reduction in the length of optimal communication due to interaction; in particular, two-sided Slepian-Wolf compression is strictly suboptimal.

==> Macro-by-Shun.tex <==
%%%%% Some Macro %%%%%%%%%%%%%%%%%%
\newcommand{\hashfunc}{f}
\newcommand{\Hash}{\mathsf{hash}}
\newcommand{\hash}{{\cal F}}

\newcommand{\Sim}{\mathsf{sim}}
\newcommand{\hQxy}{h_{\bQQ{X|Y}}(x|y)}
\newcommand{\hQXY}{h_{\bQQ{X|Y}}(X|Y)}
\newcommand{\hPxy}{h_{\bPP{X|Y}}(x|y)}
\newcommand{\hPXY}{h_{\bPP{X|Y}}(X|Y)}
\newcommand{\lambdaQXYmin}{\lambda_{\bQQ{X|Y}}^{\min}}
\newcommand{\lambdaQXYmax}{\lambda_{\bQQ{X|Y}}^{\max}}
\newcommand{\DeltaQXY}{\Delta_{\bQQ{X|Y}}} 
\newcommand{\NQXY}{N_{\bQQ{X|Y}}}
\newcommand{\lambdaQXYi}{\lambda_{\bQQ{X|Y}}^{(i)}}
\newcommand{\lambdaQXYj}{\lambda_{\bQQ{X|Y}}^{(j)}}
\newcommand{\TQXYzero}{\cT_{\bQQ{X|Y}}^{(0)}}
\newcommand{\TQXYi}{\cT_{\bQQ{X|Y}}^{(i)}}
\newcommand{\TQXYj}{\cT_{\bQQ{X|Y}}^{(j)}}
\newcommand{\TQXYone}{\cT_{\bQQ{X|Y}}^{(1)}}
\newcommand{\TPXY}{\cT_{\bPP{X|Y}}}
\newcommand{\TQXY}{\cT_{\bQQ{X|Y}}}
%%
\newcommand{\DeltaQPiOneY}{\Delta_{\bQQ{\Prot_1|Y}}}
\newcommand{\NQPiOneY}{N_{\bQQ{\Prot_1|Y}}}
\newcommand{\hQPiOneYPioneX}{h_{\bQQ{\Prot_1|Y}}(\Prot_{1\cX}|Y)}
\newcommand{\TQPiOneYzero}{\cT_{\bQQ{\Prot_1|Y}}^{(0)}}
\newcommand{\lambdaQPiOneYmin}{\lambda_{\bQQ{\Prot_1|Y}}^{\min}}
%%
\newcommand{\DeltaPPiOneY}{\Delta_{\bPP{\Prot_1|Y}}}
\newcommand{\NPPiOneY}{N_{\bPP{\Prot_1|Y}}}
\newcommand{\hPPiOneYPioneX}{h_{\bPP{\Prot_1|Y}}(\Prot_{1\cX}|Y)}
\newcommand{\TPPiOneYzero}{\cT_{\bPP{\Prot_1|Y}}^{(0)}}
\newcommand{\lambdaPPiOneYmin}{\lambda_{\bPP{\Prot_1|Y}}^{\min}}
%%
\newcommand{\DeltaPPiOneX}{\Delta_{\bPP{\Prot_1|X}}}
\newcommand{\NPPiOneX}{N_{\bPP{\Prot_1|X}}}
\newcommand{\TPPiOneXzero}{\cT_{\bPP{\Prot_1|X}}^{(0)}}
\newcommand{\TPPiOneXj}{\cT_{\bPP{\Prot_1|X}}^{(j)}}
\newcommand{\lambdaPPiOneXmin}{\lambda_{\bPP{\Prot_1|X}}^{\min}}
\newcommand{\hPPiOneXPioneX}{h_{\bPP{\Prot_1|X}}(\Prot_{1\cX}|X)}
\newcommand{\hPPiOneXPione}{h_{\bPP{\Prot_1|X}}(\Prot_1|X)}
%%%%%
\newcommand{\lambdaPPitXmin}{\lambda_{\bPP{\Prot_t|X \Prot^{t-1}}}^{\min}}
\newcommand{\lambdaPPitYmin}{\lambda_{\bPP{\Prot_t|Y \Prot^{t-1}}}^{\min}}
\newcommand{\lambdaPPitXmax}{\lambda_{\bPP{\Prot_t|X \Prot^{t-1}}}^{\max}}
\newcommand{\lambdaPPitYmax}{\lambda_{\bPP{\Prot_t|Y \Prot^{t-1}}}^{\max}}
\newcommand{\DeltaPPitX}{\Delta_{\bPP{\Prot_t|X\Prot^{t-1}}}}
\newcommand{\DeltaPPitY}{\Delta_{\bPP{\Prot_t|Y\Prot^{t-1}}}}
\newcommand{\NPPitX}{N_{\bPP{\Prot_t|X\Prot^{t-1}}}}
\newcommand{\NPPitY}{N_{\bPP{\Prot_t|Y\Prot^{t-1}}}}
\newcommand{\TPPitXzero}{\cT_{\bPP{\Prot_t|X\Prot^{t-1}}}^{(0)}}
\newcommand{\TPPitYzero}{\cT_{\bPP{\Prot_t|Y\Prot^{t-1}}}^{(0)}}

